Reverse AD at Higher Types: Pure, Principled and Denotationally Correct

We show how to define forward- and reverse-mode automatic differentiation source-code transformations or on a standard higher-order functional language. The transformations generate purely functional code, and they are principled in the sense that their definition arises from a categorical universal property. We give a semantic proof of correctness of the transformations. In their most elegant formulation, the transformations generate code with linear types. However, we demonstrate how the transformations can be implemented in a standard functional language without sacrificing correctness. To do so, we make use of abstract data types to represent the required linear types, e.g. through the use of a basic module system.

==> appx-applied-equations.tex <==
\sqsection{Equations for the Applied Target Language}\label{appx-applied-equations}
The implementation of this API is intended to respect the following equations (in contextual equivalence):
\begin{align*}
&\zero + \trm = \trm\quad \trm+\zero = \trm \quad \trm+\trm[2] = \trm[2]+\trm
\quad \trm+(\trm[2]+\trm[3])=(\trm+\trm[2])+\trm[3]
\\ 
&
\zero\lcomp\trm =\zero \quad \trm\lcomp\zero = \zero\quad
(\trm+\trm[2])\lcomp\trm[3]=(\trm\lcomp\trm[2])+(\trm\lcomp\trm[3])
\quad 
\trm\lcomp (\trm[2]+\trm[3]) = (\trm\lcomp\trm[2])+(\trm\lcomp\trm[3])\\
&\linearid\lcomp\trm=\trm\quad
\trm\lcomp\linearid =\trm\quad 
\trm\lcomp(\trm[2]\lcomp\trm[3])=(\trm\lcomp\trm[2])\lcomp\trm[3]\\ &
\lswap\, (\inv\lswap\trm)=\trm\quad \inv\lswap(\lswap\,\trm)=\trm
\quad\lcurry\,(\inv\lcurry\trm)=\trm \quad \inv\lcurry(\lcurry\,\trm)=\trm\\
&\lcurry(\trm;\trm[2])=\fun{\var}(\lcurry\,\trm\,\var);\trm[2]
\quad 
\inv\lcurry(\fun{\var}(\trm\,\var)\lcomp\trm[2])=\inv\lcurry(\trm)\lcomp\trm[2]
\\ 
&\inv\lswap(\trm;\trm[2])=\fun{\var}(\inv\lswap\,\trm\,\var);\trm[2]
\quad 
\lswap(\fun{\var}(\trm\,\var)\lcomp\trm[2])=\lswap(\trm)\lcomp\trm[2]\\
&\applin\linearid{\trm}=\trm\quad \applin{\trm\lcomp\trm[2]}{\trm[3]}=\applin{\trm[2]}{\applin{\trm}{\trm[3]}}\quad
\applin\zero{\trm}=\zero \quad \applin\trm{\zero}=\zero\\ & 
\applin{\trm+\trm[2]}{\trm[3]}=\applin{\trm}{\trm[3]}+\applin{\trm[2]}{\trm[3]}
\quad \applin{\trm}{\trm[2]+\trm[3]}=\applin{\trm}{\trm[2]}+\applin{\trm}{\trm[3]}\\
&\lPair{\trm}{\trm[2]}\lcomp\lFst=\trm\quad\! \lPair{\trm}{\trm[2]}\lcomp\lSnd=\trm[2]\quad \!
\lPair{\lFst}{\lSnd}=\linearid\quad\! \lPair{\trm\lcomp\trm[2]}{\trm\lcomp\trm[3]}=\trm\lcomp\lPair{\trm[2]}{\trm[3]}\\
\end{align*}

==> defs_arxiv.tex <==
%-- packages --
\usepackage{xcolor}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{suffix}
\usepackage{amsfonts}
\usepackage{mathpartir}
\usepackage{enumitem}
\usepackage{stmaryrd}
\usepackage[all]{xy}
\usepackage{amssymb}
\usepackage{twoopt}

\usepackage{amsthm}

%-- Theorem environments -- 

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 ##1}%
 \begin{rep@theorem}\def\@currentlabel{##1}}%
 {\end{rep@theorem}}}
\makeatother
\newreptheorem{theorem}{Theorem}
\newreptheorem{corollary}{Corollary}
\newreptheorem{proposition}{Proposition}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{corollary*}{Corollary}


%-- Syntax --
\newcommand\computationtype[1]{\underline{#1}}
\makeatletter
\newcommand\@TyAlph[1]{%
\ifcase #1\or \tau\or \sigma\or \rho\else \@ctrerr \fi%
}
\newcommand\ty[1][1]{{\@TyAlph{#1}}}

\newcommand\@CTyAlph[1]{%
\computationtype{\ifcase #1\or \tau\or \sigma\or \rho\else \@ctrerr \fi}%
}
\newcommand\cty[1][1]{{\@CTyAlph{#1}}}

\newcommand\tvar[1][1]{{\@TyVarAlph{#1}}}
\newcommand\@TyVarAlph[1]{%
\ifcase #1\or \alpha\or \beta\or \gamma\else \@ctrerr \fi%
}
\newcommand\var[1][1]{{\@VarAlph{#1}}}
\newcommand\@VarAlph[1]{%
\ifcase #1\or x\or y\or z\or u\or v\or w\else \@ctrerr \fi%
}

\newcommand\trm[1][1]{{\@TermAlph{#1}}}
\newcommand\@TermAlph[1]{%
\ifcase #1\or t\or s\or r\else \@ctrerr \fi%
}

\newcommand\val[1][1]{%
\ifcase #1\or v\or w\or u\else \@ctrerr \fi%
}

\newcommand\op[1][1]{%
\ifcase #1\or \mathsf{op}\or \mathsf{op}'\or \mathsf{op}''\else \@ctrerr \fi%
}
\makeatother
\newcommand\lop{\mathsf{lop}}
\newcommand\Op{\mathsf{Op}}
\newcommand\LOp{\mathsf{LOp}}
\newcommand\pOp{\mathsf{pOp}}
\newcommand\cnst{\underline{c}}
\newcommand\zero{\underline{0}}
\newcommand\sigmoid{\varsigma}
\newcommand\tSum{\mathrm{sum}}
\newcommand\applin[2]{\mathbf{lapp}(#1,#2)}
\newcommand\lPair[2]{\mathbf{lpair}(#1,#2)}
\newcommand\lFst{\mathbf{lfst}\,}
\newcommand\lSnd{\mathbf{lsnd}\,}
\newcommand\lcomp{;\!\!;}
\newcommand\evlin[1]{(\inv\lswap\linearid)\,#1}

\newcommand\bp[1]{\boldsymbol{(}#1\boldsymbol{)}}
\newcommand\tUnit{\tTuple{}}
\newcommand\ltUnit{\tTuple{}}
\newcommand\tPair[2]{\langle #1, #2\rangle}
\newcommand\ltPair[2]{\langle #1, #2\rangle}
\newcommand\tTriple[3]{\langle #1, #2, #3\rangle}
\newcommand\tTuple[1]{\langle #1\rangle}
\newcommand\tInj[3][\,]{#2.#3#1}
\newcommand\Cns{\ell}
\newcommand\Inj[2][\,]{\mathsf{#2}#1}
\newcommand\tNothingSym{\mathbf{nothing}}
\newcommand\tNothing[0]{\tNothingSym}
\newcommand\tJustSym{\mathbf{just}}
\newcommand\tJust[1]{\tJustSym(#1)}
\newcommand\tNil{[\,]}
\newcommand\tCons[2]{#1::#2}
\newcommand\tLeaf[1]{\mathsf{Leaf}(#1)}
\newcommand\tNode[3]{\mathsf{Node}(#1,#2,#3)}
\newcommand\tTrue{\mathbf{true}}
\newcommand\tFalse{\mathbf{false}}
\newcommand\fun[1]{\lambda #1.}
\newcommand\cfun[1]{\underline{\lambda} #1.}
\newcommand\lfun[1]{\underline{\lambda} #1.}
\newcommand\lapp[2]{#1\{#2\}}
\newcommand\letin[3]{\mathbf{let}\,#1=\,#2\,\mathbf{in}\,#3}
\newcommand\pletin[4]{\letin{\tPair{#1}{#2}}{#3}{#4}}
\newcommand\expfun[2]{\lambda #1:#2.}
\newcommand\expletin[4]{\mathbf{let}\,#1:#2=\,#3\,\mathbf{in}\,#4}
\newcommand\ifelse[3]{\mathbf{if}\,#1\,\mathbf{then}\,#2\,\mathbf{else}\,#3\,}
\newcommand\rec[2]{\mu#1.#2}
\newcommand\tRoll[2][\,]{#2.\mathbf{roll}#1}
\newcommand\tReturn[1]{\mathbf{return}\,#1}
\newcommand\tIterate{\mathbf{iterate}}
\newcommand\tSign{\mathbf{sign}}

\newcommand\lLambda{\underline{\Lambda}}
\newcommand\lev{\underline{\ev}}
\newcommand\projection{\pi}
\newcommand\injection{\iota}
\newcommand\CMon{\mathbf{CMon}}
\newcommand\DiffMon{\mathbf{Diff_{CM}}}
\newcommand\semext[1]{\{\!|#1|\!\}}

\newcommand\DiffMonNL{\mathbf{Diff_{CM}^{\mathrm{non-lin}}}}

\newcommand\tensUMatch[3][\,]{\mathbf{case}\,#2\,\mathbf{of}#1{\star}\To#3}
\newcommand\tensMatch[5][\,]{\mathbf{case}\,#2\,\mathbf{of}#1{#3}\otimes{#4}\To#5}
\newcommand\bMatch[4][\,]{\mathbf{case}\,#2\,\mathbf{of}#1!{#3}\To#4}
\newcommand\uMatch[3][\,]{\mathbf{case}\,#2\,\mathbf{of}#1\tUnit\To#3}
\newcommand\pMatch[5][\,]{\mathbf{case}\,#2\,\mathbf{of}#1\tPair{#3}{#4}\To#5}
\newcommand\tMatch[4][\,]{\mathbf{case}\,#2\,\mathbf{of}#1\tTuple{#3}\To#4}
\newcommand\vMatch[3][\,]{\mathbf{case}\,#2\,\mathbf{of}#1\{#3\}}
\newcommand\rMatch[4][\,]{\mathbf{case}\,#2\,\mathbf{of}#1\mathbf{roll}\,#3\To#4}
\newcommand\lFold[5]{\mathbf{fold}\, (#1,#2).#3\,\mathbf{over}\,#4\,\mathbf{from}\,#5}
\newcommand\tFold[7]{\mathbf{fold}_\TreeSym\, (#1,#2,#3).#4\,\mathbf{over}\,#5\,\mathbf{from}\,#6.#7}

\newcommand\tfold[2][\,]{#2.\mathbf{fold}#1}

\newcommand\tInl{\mathbf{inl}\,}
\newcommand\tInr{\mathbf{inr}\,}
\newcommand\tFst{\mathbf{fst}\,}
\newcommand\tSnd{\mathbf{snd}\,}

\newcommand\self[1]{\mathsf{self}(#1)}
\newcommand\Cat{\mathbf{Cat}}

\newcommand\ctx{\Gamma}
\newcommand\tinf{\vdash}
\newcommand\Ginf[3][]{\ctx #1\tinf #2 : #3}
\newcommand\subst[2]{#1{}[#2]}
\newcommand\sfor[2]{^{#2}\!/\!_{#1}}


\newcommand\nat{\mathbf{nat}}
\newcommand\creals{\underline{\mathbf{real}}}
\newcommand\reals{\mathbf{real}}
\newcommand\bool{\mathbf{bool}}
\newcommand\Unit{\mathbf{1}}
\newcommand\Variant[1]{\{ #1 \}}
\WithSuffix\newcommand\t*{\boldsymbol{\mathop{*}}}
\newcommand\MaybeSym{\mathbf{maybe}}
\newcommand\ListSym{\mathbf{List}}
\newcommand\semMap[2]{\mathrm{Map}[#1,#2]}
\newcommand\MapSym{\mathbf{Tens}}
\newcommand\TreeSym{\mathbf{tree}}
\newcommand\Maybe[1]{\MaybeSym(#1)}
\newcommand\List[1]{\ListSym(#1)}
\newcommand\Map[2]{\MapSym(#1,#2)}
\newcommand\LinFunSym{\mathbf{LFun}}
\newcommand\LinFun[2]{\LinFunSym(#1,#2)}
\newcommand\Tree[1]{\TreeSym(#1)}
\newcommand\To{\to}
\newcommand\nProd[0]{\Unit}
\newcommand\uProd[1]{\bp{#1}}
\newcommand\bProd[2]{\bp{#1 \t* #2}}
\newcommand\tProd[3]{\bp{#1 \t* #2 \t* #3}}
\newcommand\EmptyList{\mathbf{[\,]}}
\newcommand\EmptyMap{\mathbf{\{\,\}}}
\newcommand\PlusMap[2]{#1\oplus #2}
\newcommand\ListCons[2]{#1:: #2}
\newcommand\PlusList[2]{#1+\!\!+\, #2}
\newcommand\ListFold[5]{\mathbf{fold}\,#1\,\mathbf{over}\,#2\,\mathbf{in}\,#3\,\mathbf{from}\,#4=#5}
\newcommand\ExplicitMap[1]{\mathbf{\{}#1\mathbf{\}}}
\newcommand\SingletonMap[2]{\mathbf{\{}(#1, #2)\mathbf{\}}}
\newcommand\SetMap[3]{\mathbf{set}\,#1\mapsto#2\,\mathbf{in}\,#3}
\newcommand\FindMap[2]{\mathbf{find}\,#1\,\mathbf{in}\,#2}
\newcommand\FindMapZ[3]{\mathbf{find}^{#1}_{\zero}\,#2\,\mathbf{in}\,#3}
\newcommand\FoldMap[6]{\mathbf{fold}\,#1\,\mathbf{with}\,#2\mapsto#3\,\mathbf{in}\,#4\,\mathbf{from}\,#5=#6}
\newcommand\SumFoldMap[5][]{\mathbf{sum}_{#1}\,#2\,\mathbf{over}\,#5}

\newcommand\LDsynsymbol[1][]{\scalebox{0.8}{$\overrightarrow{\mathcal{LD}}$}_{#1}}%{{\stackrel{\to}{\mathcal{D}}}_{#1}}
\newcommand\Dsynsymbol[1][]{\scalebox{0.8}{$\overrightarrow{\mathcal{D}}$}_{#1}}%{{\stackrel{\to}{\mathcal{D}}}_{#1}}
\newcommand\Dsyn[2][]{\Dsynsymbol[#1](#2)}
\newcommand\DsynV[2][]{\Dsynsymbol[#1]{}_{\cat{V}}(#2)}
\newcommand\DsynC[2][]{\Dsynsymbol[#1]{}_{\cat{C}}(#2)}

\newcommand\LDsynrevsymbol[1][]{\scalebox{0.8}{$\overleftarrow{\mathcal{LD}}$}_{#1}}%{{\stackrel{\leftarrow}{\mathcal{D}}}_{#1}}
\newcommand\Dsynrevsymbol[1][]{\scalebox{0.8}{$\overleftarrow{\mathcal{D}}$}_{#1}}%{{\stackrel{\leftarrow}{\mathcal{D}}}_{#1}}
\newcommand\Dsynrev[2][]{\Dsynrevsymbol[#1](#2)}


\newcommand\LDcatsymbol[1][]{\scalebox{0.8}{$\overrightarrow{\mathfrak{D}}$}_{#1}}%{{\stackrel{\to}{\mathcal{D}}}_{#1}}
\newcommand\LDcatrevsymbol[1][]{\scalebox{0.8}{$\overleftarrow{\mathfrak{D}}$}_{#1}}%{{\stackrel{\leftarrow}{\mathcal{D}}}_{#1}}
\newcommand\LDcat[2][]{\LDcatsymbol[#1][#2]}
\newcommand\LDcatrev[2][]{\LDcatrevsymbol[#1][#2]}


\newcommand\Dcatsymbol[1][]{\scalebox{0.8}{$\overrightarrow{\mathfrak{D}}$}_{#1}}%{{\stackrel{\to}{\mathcal{D}}}_{#1}}
\newcommand\Dcatrevsymbol[1][]{\scalebox{0.8}{$\overleftarrow{\mathfrak{D}}$}_{#1}}%{{\stackrel{\leftarrow}{\mathcal{D}}}_{#1}}
\newcommand\Dcat[2][]{\Dcatsymbol[#1][#2]}
\newcommand\Dcatrev[2][]{\Dcatrevsymbol[#1][#2]}

\newcommand\Dnsynsymbol[1][]{\scalebox{0.8}{${\mathcal{D}}$}_{#1}}%{{\stackrel{\to}{\mathcal{D}}}_{#1}}
\newcommand\Dnsyn[2][]{\Dnsynsymbol[#1](#2)}

\newcommand\LSyn{\mathbf{LSyn}}
\newcommand\Syn{\mathbf{Syn}}
\newcommand\SynV{\Syn_\cat{V}}
\newcommand\SynC{\Syn_\cat{C}}
\newcommand\SynJ{\Syn_\cat{J}}
\newcommand\Conv{\mathbf{Conv}}


\newcommand\tNn[2]{\mathrm{nn}_{#1,#2}}
\newcommand\tlNn[2]{\mathrm{lnn}_{#1,#2}}
\newcommand\tolNn[2]{\mathrm{mlnn}_{#1,#2}}
\newcommand\tFromMaybe[1]{\mathrm{fromMaybe}}%_{#1}}
\newcommand\tFromMayben[2]{\mathrm{fromMaybe}^{#2}}
\newcommand\tInnerprod[1]{\mathrm{prod}_{#1}}
\newcommand\tSigLayer[1]{\mathrm{siglayer}_{#1}}
\newcommand\tStack[4]{\mathrm{stack}_{#1,#2}^{#3,#4}}
\newcommand\NeurN[2]{\mathbf{NeurN}_{#1}^{#2}}
\newcommand\lNeurN[2]{\mathbf{lNeurN}_{#1}^{#2}}
\newcommand\tMap{\mathbf{map}}

\newcommand{\plots}[1]{\mathcal{P}_{#1}}
%\newcommand\tMap{\mathbf{map}}
\newcommand\freeeq[1]{\stackrel{\# #1}{=}}
\newcommand\beeq{\stackrel{\beta\eta}{=}}
\newcommand\bepeq{\!\stackrel{\beta\eta+}{=}\!}


\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\ignorespaces\fi}
\makeatother

\newcommand\explainr[1]{&\pushright{\color{gray}\scriptsize\{\;\textnormal{#1}\;\}}}


%%%%%%%%%% Colors %%%%%%%%%%%%

% grey shading

\definecolor{shade}{RGB}{223,223,223}
\definecolor{unshade}{RGB}{255,255,255}

\usepackage{tcolorbox}
\newtcbox{\shadebox}{on line,arc=1pt, outer arc=2pt,%
  colback=shade,colframe=shade,boxsep=0pt,%
  left=1pt,right=1pt,top=2pt,bottom=2pt,%
  boxrule=0pt,bottomrule=1pt,toprule=1pt}
\newcommand{\shade}[1]{%
        \shadebox{\ensuremath{#1}}%
}
\newtcbox{\unshadebox}{on line,arc=1pt, outer arc=2pt,%
  colback=unshade,colframe=shade,boxsep=0pt,%
  left=1pt,right=1pt,top=2pt,bottom=2pt,%
  boxrule=0pt,bottomrule=1pt,toprule=1pt}
\newcommand{\unshade}[1]{%
        \unshadebox{\ensuremath{#1}}%
}


%%%%% Syntax
\newcommand\syncat[1]{\mspace{-25mu}\synname{#1}}
\newcommand\synname[1]{\qquad\text{#1}}

\newenvironment{syntax}[1][]{%
\(
  %\rowcolors{100}{white}{white}%
  \begin{array}[t]{#1l@{\quad\!\!}*3{l@{}}@{\,}l}
}{
\end{array}
\)%
}

\newenvironment{sugar}{%
  \(
  \begin{array}[t]{@{\bullet\ }l@{\mspace{25mu}}ll}
    \multicolumn{1}{@{\hphantom{\bullet}}l}{\text{Sugar}} & \text{Elaboration}\\
    \hline
}{
  \end{array}
  \)%
}

\newcommand\gdefinedby{::=}
\newcommand\gor{\mathrel{\lvert}}


\newcommand\vor{\mathrel{\big\lvert}}

%-- Semantics --
\newcommand{\dif}{\mathop{}\!\mathrm{d}}
\newcommand{\Diff}{\mathbf{Diff}}
\newcommand{\wDiff}{\mathbf{\omega Diff}}
\newcommand{\wCpo}{\mathbf{\boldsymbol\omega CPO}}
\newcommand{\wcpo}{$\omega$-cpo}
\newcommand{\wcpos}{$\omega$-cpos}
\newcommand{\wchain}{$\omega$-chain}
\newcommand{\wchains}{$\omega$-chains}
\newcommand\opposite[1]{#1^{\mathrm{op}}}
\newcommand\wopchain{$\opposite\omega$-chain}
\newcommand\wopchains{$\opposite\omega$-chains}
\newcommand\prj[1]{#1^{\mathrm{p}}}
\newcommand\emb[1]{#1^{\mathrm{e}}}
\newcommand\lub{\bigvee}
\newcommand\Union{\bigcup}
\makeatletter
% adapted from mathtools.sty
\def\MTrightharpoonupfill{%
  \arrowfill@\relbar\relbar\rightharpoonup}
\def\MTleftharpoondownfill{%
  \arrowfill@\leftharpoondown\relbar\relbar}
\def\MTleftharpoonupfill{%
  \arrowfill@\leftharpoonup\relbar\relbar}
\def\MTrightharpoondownfill{%
  \arrowfill@\relbar\relbar\rightharpoondown}
\newcommand*\xhookrightleftharpoons[2][]{\mathrel{%
  \raise.22ex\hbox{%
    $\lhook\joinrel\ext@arrow 0359\MTrightharpoonupfill{\phantom{#1}}{#2}$}%
  \setbox0=\hbox{%
    $\ext@arrow 3095\MTleftharpoondownfill{#1}{\phantom{\lhook\joinrel#2}}$}%
  \kern-\wd0 \lower.22ex\box0}}
\newcommand*\xleftrighthookharpoons[2][]{\mathrel{%
  \raise.22ex\hbox{%
    $\ext@arrow 3095\MTleftharpoonupfill{\phantom{#1\mspace{15mu}}}{#2}$}%
  \setbox0=\hbox{%
    $\mathrel{\raise-.4837ex\hbox{$\lhook$}}\joinrel\ext@arrow 0359\MTrightharpoondownfill{#1}{\phantom{#2}}$}%
  \kern-\wd0 \lower.22ex\box0}}
\makeatother
\newcommand\xepto{\xhookrightleftharpoons}
\newcommand\xpeto{\xleftrighthookharpoons}
\newcommand\pair[2]{\parent{#1, #2}}
\newcommand\parent[1]{\left(#1\right)}
\WithSuffix\newcommand\pair-[2]{(#1, #2)}
\newcommand\epto{\xepto{\hphantom{a}}}
\newcommand\peto{\xpeto{\hphantom{a}}}
\usepackage[bbgreekl]{mathbbol}
\newcommand\compose{\circ}
\newcommand\andthen{\mathbin;}
\newcommand{\lUnit}{\underline{\Unit}}
\newcommand{\Zero}{\mathbf{0}}
\newcommand{\lp}{\oplus}
\newcommand\diagram[1]{\begin{center}\includegraphics{diagram-#1.mps}\end{center}}
\newcommand{\Open}{\mathbf{Open}}
\newcommand{\Sh}{\mathbf{Sh}}
\newcommand{\CartSp}{\mathbf{CartSp}}
\newcommand{\Man}{\mathbf{Man}}
\newcommand{\CTop}{\mathbf{Top}}
\newcommand{\Set}{\mathbf{Set}}
\newcommand\pMap[1]{\Category{p}{#1}}
\newcommand\dmon[1][]{\partial_{#1}}
\newcommand\dfun[1]{\underline{#1}}
\newcommand\dom[1][]{D_{#1}}
\newcommand\Opens[1]{\Ocal_{#1}}
\newcommand\inv[1]{#1^{-1}}
\WithSuffix\newcommand\inv+[1]{\parent{#1}^{-1}}
\newcommand\restrict[2]{\left.#1\vphantom{\big(}\right|_{#2}}
\newcommand\initial{\mathbb{0}}
\newcommand\terminal{\mathbb{1}}
\newcommand\definedby{:=}
\newcommand\isomorphic\cong
\newcommand\intersect{\cap}
\newcommand\pto{\rightharpoonup}
\newcommand\pfrom{\leftharpoonup}
\newcommand\LS{\mathbf{LS}}
\newcommand\xpto{\xrightharpoonup}
\newcommand\Fn{\mathbf{Fn}}
\newcommand\tot{\mathop{\downarrow}\nolimits}
\newcommand\Lift[1]{#1_{\bot}}
\newcommand\RLift[1]{#1_{\tilde{\bot}}}
\newcommand\Lei{\mathbf{Leibniz}}
\newcommand{\sem}[1]{\llbracket #1\rrbracket}
\newcommand{\semgl}[1]{\llparenthesis #1\rrparenthesis^f}
\newcommand{\semglrev}[1]{\llparenthesis #1\rrparenthesis^r}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand\cat[1]{\mathcal{#1}}
\newcommand\catC{\cat{C}}
\newcommand\catD{\cat{D}}
\newcommand\catE{\cat{E}}
\newcommand\prtl{\mathbf{p}}
\newcommand\embed{\hookrightarrow}
\newcommand\freeF{F}
\newcommand\Hom{\mathrm{Hom}}
\newcommand\interpR{\sem{-}}

\newcommand\sIt{\mathsf{iterate}}
\newcommand\iterate[1]{\sIt(#1)}
\newcommand\sSign{\mathsf{sign}}
\newcommand\sInl{\mathsf{inl}}
\newcommand\sInr{\mathsf{inr}}

\newcommand{\bind}{\mathrel{\scalebox{0.8}[1]{\(>\!\!>\!=\)}}}
\newcommand{\klcomp}{\mathrel{\scalebox{0.8}[1]{\(>\!=\!>\)}}}
\newcommand{\return}[1][{}]{{\rm return}_{#1}}

\newcommand{\strength}{\mathrm{strength}}
\newcommand{\assoc}{\mathrm{assoc}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand\Dsemsymbol[1][]{\mathcal{T}^{#1}}%{\stackrel{\to}{\mathcal{T}}}
\newcommand\Dsem[2][]{\Dsemsymbol[#1](#2)}
\newcommand\Dsemrevsymbol[1][]{\mathcal{T}^*{}^{#1}}
\newcommand\Dsemrev[2][]{\Dsemrevsymbol[#1](#2)}
\newcommand\ev[1][]{\mathrm{ev}^{#1}}
\newcommand\evRsymbol[1][]{\mathrm{evR}^{#1}}
\newcommandtwoopt\evR[3][][]{\evRsymbol[#2]_{#1}(#3)}
\newcommand\lamRsymbol[1][]{\mathrm{lamR}^{#1}}
\newcommandtwoopt\lamR[3][][]{\lamRsymbol[#2]_{#1}(#3)}

\newcommand{\Gl}[1][]{\scalebox{0.8}{$\overrightarrow{\mathbf{SScone}}$}_{#1}}
\newcommand{\GlRev}[1][]{\scalebox{0.8}{$\overleftarrow{\mathbf{SScone}}$}_{#1}}

\newcommand{\Ocal}{\mathcal{O}}

\newcommand{\sPair}[2]{( #1, #2 )}
\newcommand{\sTriple}[3]{(#1, #2, #3)}
\newcommand{\sTuple}[1]{(#1)}
\newcommand{\inl}{\mathrm{inl}}
\newcommand{\inr}{\mathrm{inr}}
\newcommand\transpose[1]{{#1}^{t}}


\newcommand\leval[1]{{\mathbf {leval}}_{#1}}
\newcommand\lsing[1]{\{(#1,-)\}}
\newcommand\lcurry[1][{}]{{\mathbf {lcur}}_{#1}}
\newcommand\lswap[1][{}]{{\mathbf {lswap}}_{#1}}
\newcommand\linearid[1][{}]{{\mathbf {lid}}_{#1}}
\newcommand\id[1][{}]{{\rm id}_{#1}}
\newcommand\projsyn{\pi_{\Syn}}
\newcommand\projf{\mathrm{proj}}

\newcommand\xto\xrightarrow
\newcommand\glD{\stackrel{\to}{\mathfrak{D}}}
\newcommand\glDrev{\stackrel{\leftarrow}{\mathfrak{D}}}

\newcommand\DtoT[2][]{\phi_{#2#1}^{\Dsynsymbol\Dsemsymbol}}
\newcommand\TtoD[2][]{\phi_{#2#1}^{\Dsemsymbol\Dsynsymbol}}
\newcommand\DtoTrev[2][]{\phi_{#2#1}^{\Dsynrevsymbol\Dsemrevsymbol}}
\newcommand\TtoDrev[2][]{\phi_{#2#1}^{\Dsemrevsymbol\Dsynrevsymbol}}
\newcommand\DsemrevtoDsem[1]{\phi_{#1}^{\Dsemrevsymbol\Dsemsymbol}}
\newcommand\DsemtoDsemrev[1]{\phi_{#1}^{\Dsemsymbol\Dsemrevsymbol}}


\newcommand\Cinfty{\mathcal{C}^\infty}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.6}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\newcommand\innerprod[2]{#1\bigcdot #2}
\newcommand\sFst{\mathsf{fst}}
\newcommand\sSnd{\mathsf{snd}}
\newcommand\y{\mathbf{y}}

\newcommand\seq[2][]{\left(#2\right)_{#1}}
\newcommand\coseq[2][]{\left[#2\right]_{#1}}
\newcommand\set[1]{\left\{#1\right\}}
\newcommand\carrier[1]{\left\lvert#1\right\rvert}


\newcommand\characteristic[1]{{\rm\bf1}_{#1}}
\newcommand\Image[1]{{\rm Im}\parent{#1}}
\newcommand\Domain[1]{\mathop{\rm Dom}\parent{#1}}
\newcommand\Codomain[1]{\mathop{\rm Cod}\parent{#1}}

\newcommand\proj[1]{\pi_{#1}}
\newcommand\inj[1]{\iota_{#1}}
\newcommand\cover{\mathcal{U}}

\newcommand\colim{\mathrm{colim}}
\renewcommand\lim{\mathrm{lim}}

\newcommand\Powerset{\mathcal{P}}

\newcommand\ob[1]{\mathrm{ob}\,#1}
\renewcommand\circ{
  \PackageError{Matthijs}{Please use ; instead! Or if you'd rather use circ consistently, tell me and we'll switch the whole document over}{}}

\newcommand{\defeq}{\stackrel {\mathrm{def}}=}

%-- TODO notes --
\usepackage{todonotes}
\newcommand{\OK}[1]{\todo[inline,author=OK]{#1}}
\newcommand{\ok}[1]{\todo[size=\tiny]{OK: #1}{}}
\newcommand{\SSS}[1]{\todo[inline,author=SS]{#1}}
\newcommand{\sss}[1]{\todo[size=\tiny]{SS: #1}{}}
\newcommand{\MV}[1]{\todo[inline,author=MV]{#1}}
\newcommand{\mv}[1]{\todo[size=\tiny]{mv: #1}{}}
\newcommand{\MH}[1]{\todo[inline,author=MH]{#1}}
\newcommand{\mh}[1]{\todo[size=\tiny]{mh: #1}{}}

\makeatletter
\RequirePackage{zref}

\zref@newprop{oktheoremfreetext}{\oktheorem@parameter}

\newcommand\OKTheoremAddReferences[2]{
  \expandafter\newcommand\csname#1ref\endcsname[1]{#2~\ref{#1:##1}}
  \expandafter\newcommand\csname#1label\endcsname[1]{\label{#1:##1}}
  \WithSuffix\expandafter\newcommand\csname#1ref\endcsname*[1]{\ref{#1:##1}}
  \WithSuffix\expandafter\newcommand\csname#1label\endcsname+[1]{\hypertarget{#1+:##1}{}\zref@labelbyprops{#1:##1}{oktheoremfreetext}}
  \WithSuffix\expandafter\newcommand\csname#1ref\endcsname+[1]{\hyperlink{#1+:##1}{{{\let\ref\@refstar#2~\zref@extract{#1:##1}{oktheoremfreetext}}}}}
  \WithSuffix\expandafter\newcommand\csname#1ref\endcsname-[1]{\hyperlink{#1+:##1}{{\let\ref\@refstar{\zref@extract{#1:##1}{oktheoremfreetext}}}}}
}
\makeatother
\theoremstyle{definition}
%\newtheorem{exampleEnv}{Example}
%\newtheorem*{exampleEnv*}{Example}
%\newtheorem*{exampleEnv+}{Example \oktheorem@parameter}
%\newenvironment{example}{\begin{exampleEnv}}{\qed\end{exampleEnv}}
%\newenvironment{example*}{\begin{exampleEnv*}}{\qed\end{exampleEnv*}}
%\newenvironment{example+}[1]{\def\oktheorem@parameter{#1}\begin{exampleEnv+}}{\qed\end{exampleEnv+}}
%\OKTheoremAddReferences{example}{Example}




\newenvironment{tightitemize}{\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]}{\end{itemize}\ignorespacesafterend}
\newenvironment{tightenumerate}{\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]}{\end{enumerate}\ignorespacesafterend}

  \renewcommand\Domain[1]{\mathbf{Dom}(#1)}
  \newcommand\LDomain[1]{\mathbf{LDom}(#1)}

\newcommand\ct[1]{\underline{#1}}
\newcommand\cRR{\ct{\RR}}
\newcommand\cNN{\ct{\NN}}



==> list-type-system.tex <==
\[
  \begin{array}{c}
    \inferrule{~}{\Ginf \EmptyList {\List\ty}}
    \quad 
    \inferrule{\Ginf \trm\ty\quad \Ginf{\trm[2]}{\List\ty}}{\Ginf{\ListCons{\trm}{\trm[2]}}{\List\ty}}
    \quad 
    \inferrule{\Ginf[{,\var:\ty,\var[2]:\ty[2]}]{\trm}{\ty[2]}\quad 
    \Ginf{\trm[2]}{\List\ty}\quad 
    \Ginf{\trm[3]}{\ty[2]}
    }
    {\Ginf {\ListFold{\trm}{\var}{\trm[2]}{\trm[3]}{\var[2]}}{\ty[2]}}
    % \\ 
    % \\ 
    % \inferrule{~}{
    % \Ginf \tNothing{\Maybe\ty}}\quad\!
    % \inferrule{\Ginf \trm \ty}{
    % \Ginf {\tJust\trm} {\Maybe\ty}}\quad\!
    % \inferrule{\Ginf \trm {\Maybe\ty} \quad 
    % \Ginf{\trm[2]} {\ty[2]} \quad
    % \Ginf[,\var:\ty]{\trm[3] } {\ty[2]} 
    % }{\Ginf {\vMatch{\trm}{\tNothing\to\trm[2]\mid \tJust \var \To \trm[3]}}{\ty[2]}}
\end{array}
\]


==> practical-macro-backup.tex <==

\sqsubsection{AD Macros Targeting our New Language}
Assume that we have chosen suitable terms 
$\var:\Domain{\op}\vdash D\op(\var):\LinFun(\Domain{\op},\reals^m)$
and $\var:\Domain{\op}\vdash\transpose{D\op}(\var):\LinFun(\reals^m,\Domain{\op})$
for representing the forward and reverse derivatives of operations
$\op\in\Op_{n_1,\ldots,n_k}^m$.

For forward AD, each type $\ty$, gets translated into a pair of types 
$(\Dsyn{\ty}_1,\Dsyn{\ty}_2)$.
Each term $\var:\ty\vdash \trm:\ty[2]$ gets translated into a pair of terms 
$\var:\Dsyn{\ty}_1\vdash \Dsyn{\trm}_1:\Dsyn{\ty}_1$ and 
$\var:\Dsyn{\ty}_1\vdash \Dsyn{\trm}_2:\LinFun{\Dsyn{\ty}_2}{\Dsyn{\ty[2]}_2}$.
We then define $\Dsyn{-}$ on types as 
\begin{align*}
    &\Dsyn{\reals^n}_1 \defeq \reals^n
    && {\Dsyn{\reals^n}_2} \defeq \reals^n\\
&\Dsyn{\Unit}_1 \defeq \Unit 
&& {\Dsyn{\Unit }_2} \defeq \Unit \\
&\Dsyn{\ty\t*\ty[2]}_1 \defeq \Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1
&& \Dsyn{\ty\t*\ty[2]}_2 \defeq  \Dsyn{\ty}_2\t*\Dsyn{\ty[2]}_2\\
&\Dsyn{\ty\To\ty[2]}_1 \defeq \Dsyn{\ty}_1\To(\Dsyn{\ty[2]}_1\t* \LinFun{\Dsyn{\ty}_2}{\Dsyn{\ty[2]}_2})
&& \Dsyn{\ty\To\ty[2]}_2 \defeq  \Dsyn{\ty}_1 \To\Dsyn{\ty[2]}_2.
\end{align*}
On programs, we define it as 
\begin{align*}
&\Dsyn{\op}_1\defeq \op\\
& \Dsyn{\op}_2\defeq \var\vdash D\op(\var)\\
&\Dsyn{\id[\ty]}_1\defeq \var:\Dsyn{\ty}_1\vdash \var:\Dsyn{\ty}_1\\
&\Dsyn{\id[\ty]}_2\defeq \linearid:\LinFun{\Dsyn{\ty}_2}{\Dsyn{\ty}_2}\\
&\Dsyn{\trm;\trm[2]}_1 \defeq \var:\Dsyn{\ty}_1\vdash \subst{\Dsyn{\trm[2]}_1}
{\sfor{\var[2]}{\Dsyn{\trm}_1}}:\Dsyn{\ty[3]}_1\\
&\qquad\textnormal{where }
\var:\Dsyn{\ty}_1\vdash \Dsyn{\trm}_1:\Dsyn{\ty[2]}_1\textnormal{ and }
\var[2]:\Dsyn{\ty[2]}_1\vdash \Dsyn{\trm[2]}_1:\Dsyn{\ty[3]}_1\\
&\Dsyn{\trm;\trm[2]}_2 \defeq 
\var_1:\Dsyn{\ty}_1\vdash \Dsyn{\trm}_2\lcomp\subst{\Dsyn{\trm[2]}_2}{\sfor{\var[2]_1}{\Dsyn{\trm}_1}}:\LinFun{\Dsyn{\ty[1]}_2}{\Dsyn{\ty[3]}_2}\\
&\qquad\textnormal{where }
\var_1:\Dsyn{\ty}_1\vdash \Dsyn{\trm}_2:\LinFun{\Dsyn{\ty[1]}_2}{\Dsyn{\ty[2]}_2}
\textnormal{ and }
\var[2]_1:\Dsyn{\ty[2]}_1\vdash \Dsyn{\trm[2]}_2:\LinFun{\Dsyn{\ty[2]}_2}{\Dsyn{\ty[3]}_2}\\
&\Dsyn{\tUnit_{\ty}}_1 \defeq \_ :\Dsyn{\ty}_1\vdash \tUnit:\Unit\\
&\Dsyn{\tUnit_{\ty}}_2 \defeq \_ :\Dsyn{\ty}_1
\vdash \zero: \LinFun{\Dsyn{\ty}_2}{\lUnit}\\
&\Dsyn{\tPair{\trm}{\trm[2]}}_1 \defeq \tPair{\Dsyn{\trm}_1}{\Dsyn{\trm[2]}_1}\\
&\Dsyn{\tPair{\trm}{\trm[2]}}_2 \defeq \lPair{\Dsyn{\trm}_2}{\Dsyn{\trm[2]}_2}\\
&\Dsyn{\tFst_{\ty,\ty[2]}}_1 \defeq \var:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1\vdash 
\tFst\var:\Dsyn{\ty}_1 \\
&\Dsyn{\tFst_{\ty,\ty[2]}}_2 \defeq \_:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1
\vdash \lFst:\lPair{\Dsyn{\ty\t*\ty[2]}_2}{\Dsyn{\ty}_2}\\
&\Dsyn{\tSnd_{\ty,\ty[2]}}_1 \defeq \var:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1\vdash 
\tSnd\var:\Dsyn{\ty[2]}_1  \\
&\Dsyn{\tSnd_{\ty,\ty[2]}}_2 \defeq \_:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1\vdash
\lSnd:\lPair{\Dsyn{\ty\t*\ty[2]}_2}{\Dsyn{\ty[2]}_2}\\
&\Dsyn{\ev_{\ty,\ty[2]}}_1\defeq
\var: (\Dsyn{\ty}_1\To (\Dsyn{\ty[2]}_1\t* \LinFun{\Dsyn{\ty}_2}{
\Dsyn{\ty[2]}_2}))\t* \Dsyn{\ty}_1\vdash
\tFst ((\tFst\var)\,(\tSnd\var)):\Dsyn{\ty[2]}_1\\
&\Dsyn{\ev_{\ty,\ty[2]}}_2 \defeq 
\var_1: (\Dsyn{\ty}_1\To (\Dsyn{\ty[2]}_1\t* \LinFun{\Dsyn{\ty}_2}{ 
\Dsyn{\ty[2]}_2}))\t* \Dsyn{\ty}_1
\vdash\letin{\var[2]}{\tSnd \var_1}{}\\
&\qquad 
\lFst\lcomp \leval{\var[2]} +
\lSnd\lcomp (\tSnd ((\tFst\var_1)\,\var[2]))
:\LinFun{(\Dsyn{\ty}_1\To \Dsyn{\ty[2]}_2)\t* \Dsyn{\ty}_2}{\Dsyn{\ty[2]}_2}\\
&\Dsyn{\Lambda_{\ty,\ty[2],\ty[3]}(\trm)}_1 \defeq 
\var:\Dsyn{\ty}\vdash \fun{\var[2]}\tPair
{\subst{\Dsyn{\trm}_1}{\sfor{\var[3]}{\tPair{\var}{\var[2]}}}}
{\lPair{\zero}{\linearid}\lcomp\subst{\Dsyn{\trm}_2}{
    \sfor{\var[3]}{\tPair{\var}{\var[2]}}
    }}\\
&\qquad :\Dsyn{\ty[2]}_1\To 
(\Dsyn{\ty[3]}_1\t* \LinFun{\Dsyn{\ty[2]}_2}{\Dsyn{\ty[3]}_2})\\
&\Dsyn{\Lambda_{\ty,\ty[2],\ty[3]}(\trm)}_2 \defeq 
\var:\Dsyn{\ty}_1\vdash
\lswap(\fun{\var[2]}\lPair{\linearid}{\zero}\lcomp\subst{\Dsyn{\trm}_2}{\sfor{\var[3]_1}{\tPair{\var}{\var[2]}}})
:\LinFun{\Dsyn{\ty}_2}{\Dsyn{\ty[2]}_1\To\Dsyn{\ty[3]}_2}\\
&\qquad \textnormal{where }
\var[3]:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1\vdash \Dsyn{\trm}_1:\Dsyn{\ty[3]}_1\\
&\qquad \phantom{\textnormal{where }}
\var[3]:\Dsyn{\ty}_1\t*\Dsyn{\ty[2]}_1
\vdash \Dsyn{\trm}_2:\LinFun{\Dsyn{\ty}_2\t*\Dsyn{\ty[2]}_2}{\Dsyn{\ty[3]}_2}\\
\end{align*}

For reverse AD, each type $\ty$, gets translated into a pair of types 
$(\Dsynrev{\ty}_1,\Dsynrev{\ty}_2)$.
Each term $\var:\ty\vdash \trm:\ty[2]$ gets translated into a pair of terms 
$\var:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm}_1:\Dsynrev{\ty}_1$ and 
$\var:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm}_2:\LinFun{\Dsynrev{\ty[2]}_2}{\Dsynrev{\ty}_2}$.
We define $\Dsynrev{-}$ on types as 
\begin{align*}
    &\Dsynrev{\reals^n}_1 \defeq \reals^n
    && \Dsyn{\reals^n}_2 \defeq \reals^n\\
&\Dsynrev{\Unit}_1 \defeq \Unit 
&& \Dsynrev{\Unit }_2 \defeq \Unit \\
&\Dsynrev{\ty\t*\ty[2]}_1 \defeq \Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1
&& {\Dsynrev{\ty\t*\ty[2]}_2} \defeq  {\Dsynrev{\ty}_2}\t*{\Dsynrev{\ty[2]}_2}\\
&\Dsynrev{\ty\To\ty[2]}_1 \defeq \Dsynrev{\ty}_1\To(\Dsynrev{\ty[2]}_1\t* \LinFun{\Dsynrev{\ty[2]}_2}{\Dsynrev{\ty}_2})
&& {\Dsynrev{\ty\To\ty[2]}_2} \defeq  \Map{\Dsynrev{\ty}_1}{\Dsynrev{\ty[2]}_2}.
\end{align*}
On programs, we define it as 
\begin{align*}
    &\Dsynrev{\op}_1 \defeq \op\\
    & \Dsynrev{\op}_2\defeq \var\vdash 
    \transpose{D\op}(\var).\\
    &\Dsynrev{\id[\ty]}_1\defeq \var:\Dsynrev{\ty}_1\vdash \var:\Dsynrev{\ty}_1\\
    &\Dsynrev{\id[\ty]}_2\defeq \var_1:\Dsynrev{\ty}_1
    \vdash \linearid:\LinFun{\Dsynrev{\ty}_2}{\Dsynrev{\ty}_2}\\
    &\Dsynrev{\trm;\trm[2]}_1 \defeq \var:\Dsynrev{\ty}_1\vdash \subst{\Dsynrev{\trm[2]}_1}
    {\sfor{\var[2]}{\Dsynrev{\trm}_1}}:\Dsynrev{\ty[3]}_1\\
    &\qquad\textnormal{where }
    \var:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm}_1:\Dsynrev{\ty[2]}_1\textnormal{ and }
    \var[2]:\Dsynrev{\ty[2]}_1\vdash \Dsynrev{\trm[2]}_1:\Dsynrev{\ty[3]}_1\\
    &\Dsynrev{\trm;\trm[2]}_2 \defeq 
    \var_1:\Dsynrev{\ty}_1\vdash
    \subst{\Dsyn{\trm[2]}_2}{\sfor{\var[2]_1}{\Dsyn{\trm}_1}}\lcomp\Dsyn{\trm}_2
:\LinFun{\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty[1]}_2}\\
    &\qquad\textnormal{where }
    \var_1:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm}_2:\LinFun{\Dsynrev{\ty[2]}_2}{\Dsynrev{\ty[1]}_2}
    \textnormal{ and }
    \var[2]_1:\Dsynrev{\ty[2]}_1\vdash \Dsynrev{\trm[2]}_2:\LinFun{\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty[2]}_2}\\
    &\Dsynrev{\tUnit_{\ty}}_1 \defeq \_ :\Dsynrev{\ty}_1\vdash \tUnit:\Unit\\
    &\Dsynrev{\tUnit_{\ty}}_2 \defeq \_ :\Dsynrev{\ty}_1\vdash \zero: \LinFun{\lUnit}{\Dsynrev{\ty}_2}\\
    &\Dsynrev{\tPair{\trm}{\trm[2]}}_1 \defeq \tPair{\Dsynrev{\trm}_1}{\Dsynrev{\trm[2]}_1}\\
    &\Dsynrev{\tPair{\trm}{\trm[2]}}_2 \defeq
    \var_1:\Dsynrev{\ty}_1\vdash \lFst\lcomp \Dsynrev{\trm}_2+ \lSnd\lcomp\Dsynrev{\trm[2]}_2:
\LinFun{\Dsynrev{\ty[2]}_2\t*\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty}_2}\\
&\qquad \textnormal{where }\var_1:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm}_2:\LinFun{\Dsynrev{\ty[2]}_2}{\Dsynrev{\ty}_2}
\textnormal{ and }\var_1:\Dsynrev{\ty}_1\vdash \Dsynrev{\trm[2]}_2:\LinFun{\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty}_2}\\
&\Dsynrev{\tFst_{\ty,\ty[2]}}_1 \defeq \var:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1\vdash 
\tFst\var:\Dsynrev{\ty}_1 \\
&\Dsynrev{\tFst_{\ty,\ty[2]}}_2 \defeq \_:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1
\vdash\lPair{\linearid}{\zero}:\LinFun{\Dsynrev{\ty}_2}{\Dsynrev{\ty}_2\t* \Dsynrev{\ty[2]}_2}\\
&\Dsynrev{\tSnd_{\ty,\ty[2]}}_1 \defeq \var:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1\vdash 
\tSnd\var:\Dsynrev{\ty[2]}_1  \\
    &\Dsynrev{\tSnd_{\ty,\ty[2]}}_2 \defeq \_:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1
    \vdash \lPair{\zero}{\linearid}:\LinFun{\Dsynrev{\ty[2]}_2}{\Dsynrev{\ty}_2\t*\Dsynrev{\ty[2]}_2}\\
&\Dsynrev{\ev_{\ty,\ty[2]}}_1\defeq
\var:( \Dsynrev{\ty}_1\To (\Dsynrev{\ty[2]}_1\t* \LinFun{\Dsynrev{\ty[2]}_2} 
{\Dsynrev{\ty}_2}))\t* \Dsynrev{\ty}_1\vdash \tFst ((\tFst\var)\,(\tSnd\var)):\Dsynrev{\ty[2]}_1\\
&\Dsynrev{\ev_{\ty,\ty[2]}}_2 \defeq 
\var_1: (\Dsynrev{\ty}_1\To (\Dsynrev{\ty[2]}_1\t* \LinFun{\Dsynrev{\ty[2]}_2} 
{\Dsynrev{\ty}_2}))\t* \Dsynrev{\ty}_1\vdash\letin{\var[2]}{\tSnd\var_1}{}\\
&\qquad 
\lPair{\lsing{\var[2]}
    }{(\tFst\var_1)\,\var[2]}
:\LinFun{\Dsynrev{\ty[2]}_2}{\Map{\Dsynrev{\ty}_1}{\Dsynrev{\ty[2]}_2}\t* \Dsynrev{\ty}_2}\\
&\Dsynrev{\Lambda_{\ty,\ty[2],\ty[3]}(\trm)}_1 \defeq 
\var:\Dsynrev{\ty}\vdash \fun{\var[2]}\subst{\tPair
{\Dsynrev{\trm}_1}
{\Dsynrev{\trm}_2\lcomp \lSnd}}{\sfor{\var[3]}{\tPair{\var}{\var[2]}}}\\
&\qquad :\Dsynrev{\ty[2]}_1\To 
(\Dsynrev{\ty[3]}_1\t* \LinFun{\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty[2]}_2})\\
                    %from here
&\Dsynrev{\Lambda_{\ty,\ty[2],\ty[3]}(\trm)}_2 \defeq 
\var_1:\Dsynrev{\ty}_1\vdash
\inv\lcurry(\fun{\var[2]}\subst{\Dsynrev{\trm}_2}{\sfor{\var[3]}{\tPair{\var_1}{\var[2]}}})\lcomp \lFst:
\LinFun{\Map{\Dsynrev{\ty[2]}_1}{\Dsynrev{\ty[3]}_2}}{\Dsynrev{\ty}_2}\\
&\qquad \textnormal{where }
\var[3]:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1\vdash \Dsynrev{\trm}_1:\Dsynrev{\ty[3]}_1\textnormal{, }
\var[3]:\Dsynrev{\ty}_1\t*\Dsynrev{\ty[2]}_1
\vdash \Dsynrev{\trm}_2:\LinFun{\Dsynrev{\ty[3]}_2}{\Dsynrev{\ty}_2\t*\Dsynrev{\ty[2]}_2}\\
\end{align*}

==> self-dual-proofs.tex <==
\clearpage\sqsection{Proofs for \S \ref{sec:self-dualization}}\label{appx:proofs-self-dual}

\begin{proposition}
    $\Sigma_{\catC}\catL$ has terminal object 
    $\terminal=(\terminal,\terminal)$, binary product 
    $(A_1,A_2)\times (B_1,B_2)=(A_1\times B_1,A_2\times  B_2)$, and exponential $(A_1,A_2)\Rightarrow (B_1,B_2)=
    (A_1\Rightarrow  (B_1\times (A_2\multimap B_2)), A_1\Rightarrow B_2).$
    \end{proposition}
    \begin{proof}
    We have natural bijections 
    \vspace{-2pt}\\
    \resizebox{\linewidth}{!}{\parbox{\linewidth}{
    \begin{align*}
    &\Sigma_{\catC}\catL((A_1,A_2), (\terminal,\terminal))
    =
    \catC(A_1,\terminal)\times \catL(A_1)(A_2,\terminal)
    \cong\terminal\times \terminal
    \cong \terminal\explainr{$\terminal$ are terminal in $\catC$ and $\catL(A_1)$}\\
    &\\
    &\Sigma_{\catC}\catL((A_1,A_2), (B_1\times C_1,B_2\times  C_2))
    =\catC(A_1,B_1\times C_1)\times \catL(A_1)(A_2, B_2\times C_2)\hspace{-40pt}\;\\
    &\cong \catC(A_1,B_1)\times \catC(A_1,C_1)\times \catL(A_1)(A_2, B_2)\times 
    \catL(A_1)(A_2, C_2)\explainr{$\times $ are product in $\catC$ and $\catL(A_1)$}\\
    &\cong \Sigma_{\catC}\catL((A_1,A_2),(B_1,B_2))\times \Sigma_{\catC}\catL((A_1,A_2), (C_1,C_2))\hspace{-40pt}\;\\
    &\\
    &\Sigma_{\catC}\catL((A_1,A_2)\times (B_1,B_2), (C_1,C_2)) =
        \Sigma_{\catC}\catL((A_1\times B_1,A_2\times  B_2), (C_1,C_2))\hspace{-40pt}\; \\
        &=\catC(A_1\times B_1, C_1)\times \catL(A_1\times B_1)(A_2\times B_2, C_2)\\
        &\cong
        \catC(A_1\times B_1, C_1)\times \catL(A_1\times B_1)(A_2, C_2)\times  \catL(A_1\times B_1)(B_2,C_2)\explainr{$\times$ are coproducts in $\catL(A_1\times B_1)$}\\
        &\cong
        \catC(A_1\times B_1, C_1)\times \catL(A_1)(A_2, B_1\Rightarrow C_2)\times  \catL(A_1\times B_1)(B_2,C_2)
        \explainr{$\Rightarrow$-types in $\catL$}\\
        &\cong
        \catC(A_1\times B_1, C_1)\times \catL(A_1)(A_2, B_1\Rightarrow C_2)\times  \catC(A_1\times B_1,B_2\multimap C_2)
        \explainr{Cartesian $\multimap$-types}\\
        &\cong\catC(A_1\times B_1, C_1\times  (B_2\multimap C_2))\times 
        \catL(A_1)(A_2, B_1\Rightarrow C_2)\explainr{$\times$ is product in $\catC$}\\
        &\cong \catC(A_1, B_1\Rightarrow (C_1\times  (B_2\multimap C_2)))\times 
        \catL(A_1)(A_2, B_1\Rightarrow C_2)
        \explainr{$\Rightarrow$ is exponential in $\catC$}\\
        &= \Sigma_{\catC}\catL((A_1,A_2), (B_1\Rightarrow (C_1\times  (B_2\multimap C_2)), B_1\Rightarrow C_2))\\
        &= \Sigma_{\catC}\catL((A_1,A_2), (B_1,B_2)\Rightarrow (C_1,C_2)).\end{align*}\\[-22pt]
    }}\end{proof}
    \noindent We observe that
    we need $\catL$ to have biproducts (equivalently: to be $\CMon$ enriched) in order to show Cartesian closure.
    Further, we need linear $\Rightarrow$-types and Cartesian $\multimap$-types.
    
    \begin{proposition}
        $\Sigma_{\catC}\catL^{op}$ has terminal object $\terminal=(\terminal,\terminal)$, binary product
        $(A_1,A_2)\times (B_1,B_2)=(A_1\times B_1,A_2\times  B_2)$, and exponential $(A_1,A_2)\Rightarrow (B_1,B_2)=
        (A_1\Rightarrow  (B_1\times (B_2\multimap A_2)), !A_1\otimes B_2).$
        \end{proposition}
        \begin{proof}
            We have natural bijections
            \vspace{-2pt}\\
            \resizebox{\linewidth}{!}{\parbox{\linewidth}{
            \begin{align*}
                &\Sigma_{\catC}\catL^{op}((A_1,A_2), (\terminal,\terminal))
                =
                \catC(A_1,\terminal)\times \catL(A_1)(\terminal,A_2)
                \cong\terminal\times \terminal
                \cong \terminal
                \explainr{$\terminal$ terminal in $\catC$, initial in $\catL(A_1)$}\\
    &\\
            &\Sigma_{\catC}\catL^{op}((A_1,A_2), (B_1\times C_1,B_2\times  C_2))
            =\catC(A_1,B_1\times C_1)\times \catL(A_1)(B_2\times C_2,A_2)\hspace{-60pt}\;\\
            &\cong
            \catC(A_1,B_1)\times \catC(A_1,C_1)\times \catL(A_1)(B_2,A_2)\times 
            \catL(A_1)(C_2,A_2)
            \explainr{$\times $ product in $\catC$, coproduct in $\catL(A_1)$}\\
            &= \Sigma_{\catC}\catL^{op}((A_1,A_2),(B_1,B_2))\times \Sigma_{\catC}\catL^{op}((A_1,A_2), (C_1,C_2))
            \\
            &\\
                &\Sigma_{\catC}\catL^{op}((A_1,A_2)\times (B_1,B_2), (C_1,C_2)) =
                \Sigma_{\catC}\catL^{op}((A_1\times B_1,A_2\times  B_2), (C_1,C_2))\hspace{-60pt}\; \\
                &=\catC(A_1\times B_1, C_1)\times \catL(A_1\times B_1)(C_2, A_2\times B_2)\\
                &\cong
                \catC(A_1\times B_1, C_1)\times \catL(A_1\times B_1)(C_2, A_2)\times \catL(A_1\times B_1)(C_2, B_2)
                \explainr{$\times$ is product in $\catL(A_1\times B_1)$}\\
                &\cong            \catC(A_1\times B_1, C_1)\times\catC(A_1\times B_1,C_2\multimap B_2)\times 
                \catL(A_1\times B_1)(C_2, A_2)\hspace{-40pt}\;
                 \explainr{Cartesian $\multimap$-types}\\
                &\cong
                \catC(A_1\times B_1, C_1\times  (C_2\multimap B_2))\times 
                \catL(A_1\times B_1)(C_2, A_2)
                \explainr{$\times$ is product in $\catC$}\\
                &\cong
                \catC(A_1,B_1\Rightarrow ( C_1\times  (C_2\multimap B_2)))\times 
                \catL(A_1\times B_1)(C_2, A_2)
                \explainr{$\Rightarrow$ is exponential in $\catC$}\\
                &\cong
                \catC(A_1,B_1\Rightarrow ( C_1\times  (C_2\multimap B_2)))\times 
                \catL(A_1)(!B_1\otimes C_2, A_2)
                \explainr{$!(-)\otimes(-)$-types} \\
                &=
                \Sigma_{\catC}\catL^{op}((A_1,A_2), (B_1\Rightarrow ( C_1\times  (C_2\multimap B_2)), !B_1\otimes C_2))\\
                &= 
                \Sigma_{\catC}\catL^{op}((A_1,A_2), (B_1,B_2)\Rightarrow (C_1,C_2)).\\[-22pt]
            \end{align*}}}
        \end{proof}
    \noindent Observe that we need the biproduct structure of $\catL$ to construct finite products in
    $\Sigma_{\catC}\catL^{op}$.
    Further, we need Cartesian $\multimap$-types 
    and $!(-)\otimes (-)$-types to construct exponentials, but not biproducts.
